A Homological Approach to Belief Propagation and Bethe Approximations

We introduce a differential complex of local observables given a decomposition of a global set of random variables into subsets. Its boundary operator allows us to define a transport equation equivalent to Belief Propagation. This definition reveals a set of conserved quantities under Belief Propagation and gives new insight on the relationship of its equilibria with the critical points of Bethe free energy.

==> src/I/observables.tex <==
\subsection{Observables and States}

\subsubsection{Microscopic Observables.}

A microscopic observable on a region $\aa \incl \Omega$ is 
a real function on $E_\aa$.
We denote by $\obs_\aa$ the commutative algebra of observables:
\[ \obs_\aa = \R^{E_\aa} \]
For every subregion $\bb \incl \aa$, any observable $u_\bb \in \obs_\bb$ 
admits a natural extension $j_{\aa\bb}(u_\bb) \in \obs_\aa$ to $E_\aa$ defined by:
\[ j_{\aa\bb}(u_\bb)(x_\aa) = u_\bb(\pi^{\bb\aa}(x_\aa)) \]
The canonical injections $j_{\aa\bb} : \obs_\bb \aw \obs_\aa$ make
$\obs : X^{op} \aw \Alg$ a contravariant functor from $X$ to the category
of unital commutative real algebras. We note $1_\aa$ for the unit of $\obs_\aa$.

We may also view $\obs_\aa$ as the abelian Lie algebra of the multiplicative Lie group
of strictly positive observables:
\[ G_\aa = (\R^*_+)^{E_\aa} \]
We chose $u_\aa \mapsto \e^{-u_\aa}$ as prefered isomorphism between 
$\obs_\aa$ and $G_\aa$.


\subsubsection{Densities.}

A density over a region $\aa \incl \Omega$
is a linear form on observables $\omega_\aa \in \obs^*_\aa$.
We denote by $\Sigma^{\bb\aa}(\omega_\aa) \in \obs^*_\bb$ 
the density defined by
integrating $\omega_\aa$ on the fibers of $\pi^{\bb\aa}$:
\[ \Sigma^{\bb \aa}(\omega_\aa)(x_\bb) = 
\sum_{x' \in E_{\aa \setminus \bb}} \omega_\aa(x_\bb, x') \]
The canonical projection $\Sigma^{\bb\aa}:\obs^*_\aa \aw \obs^*_\bb$ is dual
to $j_{\aa\bb}$, as for every observable $u_\bb \in \obs_\bb$ 
and every density $\omega_\aa \in \obs^*_\aa$ we have:
\[ \croc{\Sigma^{\bb \aa}(\omega_\aa)}{u_\bb} 
= \croc{\omega_\aa}{j_{\aa\bb}(u_\bb)} \]
Density spaces yield a covariant functor $\obs^* : X \aw \Vect$. 

\subsubsection{Statistical States.}

A statistical state of a region $\aa \incl \Omega$ is a 
probability density on $E_\aa$. We write:
\[ \Delta_\aa = \Prob(E_\aa) \]
The convex set of statistical states $\Delta_\aa$ 
is a topological simplex of dimension
$| E_\aa | - 1$. 
In more algebraic terms, $\Delta_\aa \incl \obs^*_\aa$ is 
the set of states\footnotemark{} of the algebra of observables on $\aa$.
Its image under the continuous map $\Sigma^{\bb\aa}$ is $\Delta_\bb$
so that $\Delta : X \aw \Top$ defines a covariant functor.

The interior $\Del_\aa$ of the probability simplex on $E_\aa$
consists of all the non-vanishing probability densities. 
It is diffeomorphic to the quotient of $G_\aa$ by scalings of $\R_+^*$,
itself isomorphic to the quotient of $\obs_\aa$ by the action of additive constants.
\[ \Del_\aa \sim \P G_\aa \sim \obs_\aa / \R \]
It follows that $\Del_\aa$ has a natural Lie group structure.
The extensions $j_{\aa\bb}$ admit a quotient by scalings
and $\Del : X^{op} \aw \Grp$ also defines a contravariant functor.

Given a strictly positive observable $f_\aa \in G_\aa$, we denote by
$[f_\aa] \in \Del_\aa$ the induced normalised probability density. 
The local Gibbs state associated to an effective hamiltonian $U_\aa \in \obs_\aa$ 
is the statistical state:
\[ \rho_\aa(U_\aa) = [\e^{-U_\aa}] \]
Local Gibbs states define a natural transformation $\rho : \obs \aw \Del$.

\footnotetext{
A state of $\obs_\aa$ is a linear form $p_\aa \in \obs^*_\aa$ 
satisfying the following positivity and normalisation axioms:
$\croc{\omega_\aa}{u_\aa^2} \geq 0$ for every $u_\aa \in \obs_\aa$
and $\croc{\omega_\aa}{1_\aa} = 1$.
}


